A Large Scale Corpus of Gulf Arabic

Most Arabic natural language processing tools and resources are developed to serve Modern Standard Arabic (MSA), which is the official written language in the Arab World. Some Dialectal Arabic varieties, notably Egyptian Arabic, have received some attention lately and have a growing collection of resources that include annotated corpora and morphological analyzers and taggers. Gulf Arabic, however, lags behind in that respect. In this paper, we present the Gumar Corpus, a large-scale corpus of Gulf Arabic consisting of 110 million words from 1,200 forum novels. We annotate the corpus for sub-dialect information at the document level. We also present results of a preliminary study in the morphological annotation of Gulf Arabic which includes developing guidelines for a conventional orthography. The text of the corpus is publicly browsable through a web interface we developed for it.

==> Evaluation.tex <==
% THIS TABLE NEEDS CLEANUP __ IT IS NOT CLEAR
%\begin{table}
%\setlength{\tabcolsep}{2pt}
%\begin{center}
%\begin{footnotesize}
%\begin{tabular}{|l|c|c|c|}
%\hline
%
%\bf Input & \bf No. of Words & \bf MSA & \bf EGY\\ \hline\hline
%Raw & 4304 & 400 & 240\\ \hline
%CODA & 4401 & 230 & 105\\ \hline
%\end{tabular}
%\end{footnotesize}
%\end{center}
%\caption{Number of NO-ANALYSIS words with different inputs}
%\label{Eval_NOAN}
%\end{table}

%\paragraph{Manual Annotation}
We conduct an evaluation of the quality of automatic morphological annotation tools (taggers) on this corpus to assess the amount of effort needed to manually annotate it.
Following the annotation guidelines discussed above, we  manually annotated around 4K words from four different novels with a goal to capture different dialects, styles of writing, etc.
%\footnote{We will provide many examples and evaluation details in the camera ready that we cannot include here because of the Abstract word length limit.}
An example of an annotated sentence showed in Table~\ref{exmp_Anno}. 
%There are 143 (2.67\%) cases of merging and splitting in total, with about 80.4\% merged words and 18.2\% split words and 1.4\% of words contains merged and split parts.
As a preliminary experiment, we investigated the frequency of out-of-vocabulary (OOV) words in both systems of MADAMIRA: MSA and EGY. 
The Egyptian model OOV (5.6\%) was almost half that of MSA (9.3\%), suggesting it is better to work with Egyptian as the base system for manual annotation.
%Table~\ref{Eval_NOAN} shows the different results of the experiments. This suggests that minimum annotation of the words only might help the overall performance of automated annotation.

\begin{table*}
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{8}{|c|}{\bf MADAMIRA-EGY}\\ \hline
\multicolumn{2}{|l|}{\bf Raw} & \bf CODA & \bf ATB+Morph & \bf POS & \bf CATiB 6& \bf Lemma & \bf Gloss \\ \hline
<zyAd> & zyAd & zyAd & zyAd & noun\_prop & PROP & ziyAd & Ziad\\ \hline
: & : & : & : & punc & PNX & : & :\\ \hline
<lysA'> &lysA' & lysA' & lysA' & \cellcolor{red!25}noun & \cellcolor{red!25}NOM & \cellcolor{red!25}>aloyas\_1 & \cellcolor{red!25}valiant\\ \hline
<mysA'> & mysA' & \cellcolor{red!25}mAysA' & \cellcolor{red!25}mA+y+sA' & \cellcolor{red!25}verb & \cellcolor{red!25}VRB & \cellcolor{red!25}>asA'\_1 & \cellcolor{red!25}be\_harmed\\ \hline
<AntwlAzm> & AntwlAzm & \cellcolor{red!25}NOAN & \cellcolor{red!25}NOAN & \cellcolor{red!25}NOAN & \cellcolor{red!25}NOAN & \cellcolor{red!25}NOAN & \cellcolor{red!25}NOAN\\ \hline
<tjAbwn> & tjAbwn & \cellcolor{red!25}tjAbwn & \cellcolor{red!25}t+jAb+wn & verb & VRB & \cellcolor{red!25}>ajAb\_1 & \cellcolor{red!25}be\_answered\\ \hline
<`> & E & \cellcolor{red!25}ElY & \cellcolor{red!25}ElY & \cellcolor{red!25}prep & \cellcolor{red!25}PRT & \cellcolor{red!25}EalaY\_1 & \cellcolor{red!25}on\\ \hline
<kl> & kl & kl & kl & noun\_quant & NOM & kul{\SHADDA} & all\\ \hline
<Aly> & Aly & Ally & Ally & pron\_rel & NOM & All{\SHADDA}iy & which\\ \hline
<yqwlkm> & yqwlkm & \cellcolor{red!25}yqwlkm & \cellcolor{red!25}y+qwl+km & \cellcolor{red!25}verb & \cellcolor{red!25}VRB & \cellcolor{red!25}qAl\_1 & \cellcolor{red!25}said\\ \hline
\multicolumn{8}{c}{ }\\ \hline
\multicolumn{8}{|c|}{\bf Manual Annotation}\\ \hline 
\multicolumn{2}{|l|}{\bf Raw}  & \bf CODA & \bf ATB+Morph & \bf POS & \bf CATiB 6& \bf Lemma & \bf Gloss \\ \hline
<zyAd> & zyAd & zyAd & zyAd & noun\_prop & PROP & ziyAd & Ziad\\ \hline
: & : & : & : & punc & PNX & : & :\\ \hline
<lysA'>&  lysA' & lysA' & lysA' & \cellcolor{green!25}noun\_prop & \cellcolor{green!25}PROP & \cellcolor{green!25}laysaA' & \cellcolor{green!25}Laysaa\\ \hline
<mysA'> & mysA' & \cellcolor{green!25}mysA' & \cellcolor{green!25}mysA' & \cellcolor{green!25}noun\_prop & \cellcolor{green!25}PROP & \cellcolor{green!25}MayosaA' & \cellcolor{green!25}Maysaa\\ \hline
<AntwlAzm> & AntwlAzm & \cellcolor{green!25}Antw\#lAzm & \cellcolor{green!25}Antw\#lAzm & \cellcolor{green!25}pron\#noun & \cellcolor{green!25}NOM\#NOM & \cellcolor{green!25}Antw\#lAzim & \cellcolor{green!25}you\#necessary\\ \hline
<tjAbwn> & tjAbwn & \cellcolor{green!25}tjAwbwn & \cellcolor{green!25}t+jAwb+wn & verb & VRB & \cellcolor{green!25}jAwab & \cellcolor{green!25}comply\\ \hline
<`> & E & \cellcolor{green!25}E\# & \cellcolor{green!25}E+\# & \cellcolor{green!25}NA & \cellcolor{green!25}NA & \cellcolor{green!25}NA & \cellcolor{green!25}NA\\ \hline
<kl> & kl & kl & kl & noun\_quant & NOM & kul{\SHADDA} & all\\ \hline
<Aly> & Aly & Ally & Ally & pron\_rel & NOM & All{\SHADDA}iy & which\\ \hline
<yqwlkm> & yqwlkm & \cellcolor{green!25}yqwlh\#lkm & \cellcolor{green!25}y+qwl+h\#l+km & \cellcolor{green!25}verb\#prep & \cellcolor{green!25}VRB\#PRT & \cellcolor{green!25}qAl\#la & \cellcolor{green!25}said\#to\\ \hline 

\end{tabular}
\end{footnotesize}
\end{center}
\caption{Example of Manual Annotation}
\label{exmp_Anno}
\end{table*}

\begin{table}[h]
\setlength{\tabcolsep}{2pt}
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|c|c|}
\hline
\bf Feature & \bf MADAMIRA-MSA & \bf MADAMIRA-EGY\\ \hline\hline
CODA & 83.81 & 88.34\\ \hline
Morph & 76.16& 83.62\\ \hline
POS & 72.37 & 80.39 \\ \hline
CATiB & 76.28 & 81.51\\ \hline
Lemma & 64.03 & 77.02 \\ \hline
%\hline
%POS-subset & 73.21 & 81.46\\ \hline
%CATiB-subset  & 77.14 & 82.69\\ \hline
%lmm & 76.67 & 83.18\\ \hline
\end{tabular}
\end{footnotesize}
\end{center}
\caption{Results on evaluation of our Gold annotation against the output of MADAMIRA in both modes: MSA and EGY}
\label{Evaluation}
\end{table}


%THIS HAS NEW TEXT THAT WS NOT IN THE ORIGINAL:
%\paragraph{Evaluation against MSA and EGY}
 We evaluated using the accuracy measure for word orthography, tokenization, POS,  and lemma against the output of both models of MADAMIRA: MSA and EGY. Table~\ref{Evaluation} shows the results of the the evaluation for all words. 
 %Features POS-subset and CATiB-subset are calculated in a way to avoid penalization over merged text that the system failed to recognize, where we match for just one correct POS/CATiB from the set of annotated ones. The lmm feature is a reduced version of the Lemma where we remove all the diacritization.
%
These numbers allow us to assess the basic quality of the these tools on GA.  As expected, MADAMIRA-EGY outperforms MADAMIRA-MSA between 4 and 13\% absolute on different metrics, confirming that it is better to use it as a baseline. This is similar to results reported by \newcite{jarrar2014building} on Palestinian Arabic.


%\begin{table}
%\setlength{\tabcolsep}{2pt}
%\begin{center}
%\begin{tabular}{|l|c|}
%\hline
%\bf Source of Error & \bf Occurrences \\ \hline\hline
%Morph & 6.6 \\ \hline
%POS & 52.1 \\ \hline
%lemma & 18.2 \\ \hline
%OOV & 16.5 \\ \hline
%MRG & 3.3 \\ \hline
%SPLT & 2.5 \\ \hline
%TP & 0.8  \\ \hline
%% Proper  Noun& 20\\ \hline
%% Wrong Annotation & 2 \\ \hline
%% Hamza Annotation & 20 \\ \hline
%% Typo & 8\\ \hline
%% Lemma & 14 \\ \hline
%% Out of Vocabulary & 18 \\ \hline
%% Merged Words  & 14 \\ \hline
%% Split Words & 3 \\ \hline
%% Wrong Analysis Choice & 1 \\ \hline
%\end{tabular}
%\end{center}
%\caption{Results on Error Analysis on Evaluation against MADAMIRA-EGY}
%\label{err_analysis}
%\end{table}
\paragraph{Error Analysis}
We manually investigated the four sets of 100 words from different parts of the MADAMIRA-EGY annotated sub-corpus (total 400 words, with an average of 30 words containing at least one error).
%of each of the four annotated parts of the novels against the output of MADAMIRA-EGY. An average of 30 words errors per 100 words. Table~\ref{err_analysis} shows the percentages of different sources of errors that occurs. 
52.1\% of the errors are likely due the wrong assignment of POS especially in proper nouns that look like nouns or adjectives. Another major source of error is the lemma 18.2\% and out of vocabulary related errors are 16.5\% and this happens for two main reasons, either the word is never seen before or because of a typo. Finally, errors that come from a mistake in merging or splitting word tokens, typos and tokenization words combine around 13\%.
%
%We manually investigated the first 100 words of each of the four annotated parts of the novels against the output of MADAMIRA-EGY. An average of 30 words errors per 100 words. Table~\ref{err_analysis} shows the percentages of different sources of errors that occurs. 52.1\% of the errors are likely due the wrong assignment of POS especially in proper nouns that look like nouns or adjectives. Another major source of error is the lemma 18.2\% and out of vocabulary (OOV) related errors are 16.5\% and this happens for two main reasons, either the word is never seen before or because of a typo. Finally, errors that com from a mistake in merging (MRG) or splitting (SPLT), typos (TP) and tokenization  (Morph) words combine around 13\%.
%We manually investigated the first 100 errors of the evaluation agains the output of MADAMIRA-EGY. More than 45\% of the errors come from unseen words, that are proper nouns, out of vocabulary or writer typos. In 14\% of the time, the source of error is the presence of a different lemma, and that is caused by a number of things like changing the lemma diacritization as part of the annotaion, wrong analysis chosen by the analyzer of just out of vocabulary. Following the annotation guidelines regarding the {\it {Hamza}}, causes a total of 20\% mismatch errors. Another major source of error is words that are merged in the raw text, hence resulting in inaccurate or no answer from the analyzer, this happens 14\% of the time. On contrast to merging, splitting also happens but in a lower frequency, that is 3\%. Less common errors come from either wrong annotation 2\% or wrong analysis for no clear reason 1\%. See Table~\ref{err_analysis}

%\paragraph{Dialect Evaluation}
%
%------------------------
%
%---dialect eval? stats
%
%------------------------
